CrisisLTLSum: A Benchmark for Local Crisis Event Timeline Extraction and Summarization

Social media has increasingly played a key role in emergency response: first responders can use public posts to better react to ongoing crisis events and deploy the necessary resources where they are most needed. Timeline extraction and abstractive summarization are critical technical tasks to leverage large numbers of social media posts about events. Unfortunately, there are few datasets for benchmarking technical approaches for those tasks. This paper presents CrisisLTLSum, the largest dataset of local crisis event timelines available to date. CrisisLTLSum contains 1,000 crisis event timelines across four domains: wildfires, local fires, traffic, and storms. We built CrisisLTLSum using a semi-automated cluster-then-refine approach to collect data from the public Twitter stream. Our initial experiments indicate a significant gap between the performance of strong baselines compared to the human performance on both tasks. Our dataset, code, and models are publicly available.

==> Meeting.tex <==
 The teminology: 
Dataset name:

Dataset Creation steps:

1. Knowledge-enhanced online clustering
 --> Timeline Generation (how it differs)
2. Human Annotation
--> CrisisLTLSum Human Annotation
Tasks:
task 1: Timeline Extraction
input: Noisy Timelines
output: Clean Timeline
task 2: Timeline Summarization
input: clean timeline
output: abstractive summary


Quality experiments:
--> Agreement of 1000 timelines for task 1.
 --> All three, pairwise?
 
--> Human control of task 1 ( 133 timelines)

--> Human Sumary Qualification ( 100)


Splits:

Result report:



==> not_used/abs_old.tex <==
% This paper proposes the first dataset on local crisis event timelines extracted from Twitter. 
% We employ a two-step timeline generation and correction process to create this dataset on top of the Twitter open-access API. First, we propose an online clustering pipeline to form clusters of tweets relevant to unique local crisis events. Second, we conduct annotation tasks to remove noisy and redundant data from the generated clusters and to create timelines. To enable downstream tasks to benefit from this dataset, we introduce the timeline correction and abstractive timeline summarization tasks. This dataset is the first large-scale benchmark that provides quality summary annotation toward abstractive summarization over crisis events. Our dataset covers over a thousand unique local events in four categories: local fire, storm, wildfire, and traffic. Our experiments indicate that both the timeline correction and summarization tasks are very challenging, and there is a considerable gap between the performance of state-of-the-art models with the human performance on these tasks. 

% In this paper, we present the first dataset on crisis event timelines extracted from Twitter. The proposed dataset is generated through a semi-automated process by applying a clustering pipeline on the Twitter open access api and conducting an annotation task to clean the extracted clusters. Each cluster represents a real-life local crisis event, where each tweet in the timeline brings updates for the event. Our dataset addresses some of the challenges with the existing datasets such as noisiness and redundancy of information and further extend the scope of crisis events not only to large events but also to more local ones.
% We propose two tasks on top of this dataset, namely, Timeline Correction and Timeline Summarization. We further provide simple, yet powerful, baselines for each task. Our experiments indicate that both timeline correction and summarization tasks are very challenging and there is still a huge gap between human performance and SOTA models on this dataset. 

% Our dataset contains clusters of tweets that belong to the same real-life local event. We have annotated each cluster/timeline with additional incremental information for each tweet to be part of the timeline or not part of the timeline due to being not related to the story, being repetitive, and not having any disaster relevant information. Finally, each timeline is summarized by annotators to be used as a benchmark for twitter timeline summarization benchmark. 

==> not_used/additional.tex <==
% Timeline summarization has also been investigated in other domains such as news~\cite{nallapati2016abstractive,narayan2018don,gusev2020dataset}, Reddit~\cite{kim2018abstractive}, academic papers~\cite{lo2019s2orc}, dialogues~\cite{gliwa2019samsum}, and tutorials~\cite{koupaee2018wikihow}. Again, except some~\cite{kim2018abstractive}, most of these domains have only focused on extractive summarization.
% Additionally, summarizing timelines extracted from Twitter is more challenging due to the amount of noise~\cite{alam2021humaid}, the poor language~\cite{rudra2018extracting}, and the high overlap of information described in multiple tweets~\cite{rudra2018extracting}.
% Compared to centralized sources such as news~\cite{nallapati2016abstractive}, tweets can provide more frequent and real-time updates while covering various angles of an ongoing event.


% As the main focus of our dataset is to enable future research on real-time timeline extraction for local crisis events, 

% The importance of crisis domain information gathering and its role in understanding them
% The rise in technology has provided tools such as Twitter, which provide new sources of real-time information~\cite{hua2012information}. Such real-time information can be used to detect and track global/local events~\cite{zhang2019tracking,mamo2021fine}. This available large data source can also be used for extracting historical information for studying known events~\cite{repp2018extracting}.
% The availability of information through Twitter in the early hours of an event compared to the traditional sources is of great importance for applications in news~\cite{repp2018extracting} and crisis~\cite{martinez2018twitter} domains.
% One of the domains which can widely benefit from both real-time information and historical data is the crisis domain~\cite{}. 
% Extracting real-time crisis-related events from microblogs such as Twitter is important as it provides time-sensitive information which enables first responders to understand an ongoing situation and plan relief efforts accordingly~\cite{sarter1991situation}.
% Furthermore, extracting related information to an event can lead to benefits such as preventing future disastrous events in high-threat areas, helping first responders better understand and evaluate each event, and enabling a more profound understanding of factors and consequences of crisis events. 
% Furthermore, real-time crisis monitoring through social media can help people track an ongoing event to either provide life-saving emergency alerts, avoid getting close to the threat areas, or analyze the risks on important assets affected by the disaster.
% Tweets may contain information about the location of an event, type of the event, the severity of the situation, time of the incident, its progress, overall report, and consequences. 
% Compared to centralized sources such as news~\cite{nallapati2016abstractive}, tweets can provide more frequent and real-time updates while covering various angles of an ongoing event. However, extracting such information from Twitter is more challenging due to the amount of noise~\cite{alam2021humaid} and the poor language~\cite{rudra2018extracting}.

% Here, we provide a new dataset on concrete crisis event timelines on local events.
% Recent research has vastly investigated extracting crisis event from Twitter~\cite{alam2018crisismmd,olteanu2014crisislex,alam2021crisisbench,imran2016twitter}.
% This new dataset resolves some of the shortcomings of the existing resources and further expands the applications of such information by proposing two new tasks of timeline correction and timeline summarization.
% First, most of the prior research focuses on the extraction task as historic data~\cite{} where relevant tweets to an already known event are extracted. Here, we extract such information by relaxing this assumption by assuming no access to known events. This will help close the gap between the data generation approach and the real-life applications of such systems. Obviously, detecting and following unknown disaster events in an online system is harder due to not having access to a set of known names or keywords related to the events.

% First, existing datasets~\cite{alam2018crisismmd,alam2021crisisbench,alam2021humaid,olteanu2014crisislex,imran2016twitter} mostly focus on extracting information about known large disaster events such as long-lasting hurricanes, large earthquakes, or wildfire.
% This has imposes two major limitations. First, there is a need to have a set of curated keyword for each event individually. Second, this can only enable further understanding on very big events while crisis domain also includes a lot of smaller sized and local events. To address the first challenge, we do not start by a set of known events and instead rely on more general usage keyword lists which enables real-time detection.
% Obviously, detecting and following unknown disaster events in an online system is harder due to not having access to a set of known names or keywords, related to the events.
% To remove the second limitation, we further extend the extraction pipeline to support local events such as "a fire in a building", traffic accidents, or local wildfires by relying on location augmentation techniques. This essentially imposes a harder extraction challenge as local information appear less frequent in the tweet stream, which makes it harder for conventional clustering methods to detect them as spikes or clusters.

% Second, the extracted data in current datasets are often noisy, contain redundancy, and have overloaded information~\cite{alam2021humaid}. To address this issue, prior research~\cite{alam2021humaid} has considered fine-grained classification annotation for categorizing the tweets into groups such as prayers, urgent needs, or missing people. Although, this is a good step toward filtering out some of the noisy data, the redundancy challenge still remains open. detecting redundancy in a set of tweets is especially harder than a simple pair-based search as the information of one tweet is usually covered not by only one individual tweet but by an aggregation of multiple ones.

% The noise and duplicate removal are crucial steps on real-time tracking of events where new information should not be missed as hundreds of relevant tweets are frequently being added to the story. Here, we employ two post-processing steps to remove noise and redundancy as much as possible and later conduct an annotation task aiming to clean the clusters further. 
% The results of the annotation task can be later used on real-time extraction systems to filter out unrelated or repetitive information.

% Lastly, this is the first twitter dataset that proposes the task of abstractive summaries for crisis events and provides multiple gold annotations. Summarizing tweets are generally harder than other sources of information, given poor-language, and the the high overlap of information described in multiple tweets~\cite{rudra2018extracting}.

% Our dataset will pave the way toward extracting information about a wider range of crisis events while increasing the quality of the extractions to produce a clean and concrete timeline from microblogs in real-time while avoiding repetitive information.

% In our proposed dataset, each crisis event is called a timeline as it is represented by a chronologically sorted sequence of tweets. In contrast to the existing crisis datasets where each cluster contains every related tweet to the event, each tweet in our timelines should bring a new and important update to the story. This results in a clean timeline where the event and its progress is described clearly and is tractable. This can enable future research toward creating online systems for detecting crisis events and tracking them for updates as the event is progressing.

% We employ a two step strategy to create this dataset. First, we design an online clustering pipeline which extracts and clusters the tweet stream into a set of generated timelines. Second, we design an annotation task where a combination of experts and workers are asked to clean the generated timelines through a set of carefully designed tasks. We discuss the first step in Section \ref{sec:generate} and the annotation platform in Section \ref{sec:correct}. 
% Given the designed annotation task, we provide the following information about each tweet in the timeline. First, we specify whether each tweet belongs to the timeline. A tweet only belongs to the timeline, if it is related to the ongoing local story and provides a new information which has not been seen in any of the prior tweets. Second, if a tweet does not belong to the timeline, we provide a reason for the exclusion among not being related, not being informative, or not containing any new information.
% We further propose two tasks of timeline correction and timeline summarization in this dataset. The former task is to detect whether a tweet belongs to a given timeline and the reason of exclusion in case the tweet does not. The latter task is to generate a summary given a clean timeline of an event. 


==> sections/intro_old.tex <==
\section{Introduction}

Extracting real-time information on crisis events from microblogs such as Twitter has become an increasingly important area~\cite{zhang2019tracking,mamo2021fine} due to its role in providing time-sensitive information which can help first responders to understand ongoing situations and plan relief efforts accordingly~\cite{sarter1991situation}. Recent research has heavily investigated extracting such information from Twitter both in real-time~\cite{schulz2013see,rudra2018extracting,kumar2011tweettracker} and retrospectively~\cite{repp2018extracting,alam2021crisisbench,alam2021humaid}. Existing datasets in the crisis response domain facilitate the detection of crisis relevant tweets and mapping them to humanitarian categories~\cite{wiegmann2020disaster,imran2013practical,olteanu2014crisislex,imran2016twitter,alam2018crisismmd,alam2021crisisbench,alam2021humaid}, actionable information~\cite{mccreadie2019trec}, or specific witness levels~\cite{zahra2020automatic}. The major focus of these datasets is to extract all available information about significant disaster events such as long-lasting storms, earthquakes, and large wildfires. 

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/intro_example.pdf}
\caption{This is a sample annotated timeline from \datasetname{}. The noisy timeline is the set of tweets sorted chronologically. The first tweet is the seed of the event. \cmark~means that the tweet is annotated to be part of the timeline and \xmark~indicates that the tweet is excluded from the timeline. The reason for exclusion is written under the mark.}
\label{fig:main-example}
\end{figure}

In this paper, we propose \datasetname{}, the first dataset on concrete timelines of local crisis events extracted from Twitter and the first to provide human-written summaries on crisis event timelines. Figure \ref{fig:main-example} shows an example of an annotated timeline. A timeline is a chronologically sorted set of tweets, where each brings in new information or updates about an ongoing event. The term ``local'' is used here to indicate that the event is bound to an exact location, such as a building, a street, or a county, and usually lasts for a short period of time. This is primarily different from prior work that focused on large-scale and long-lasting crisis events affecting multiple and broader geographical areas. 
% multiple cities or states, or a whole country. 
Consequently, although most existing datasets in crisis domain are limited to only tens of unique events \cite{imran2013practical,imran2016twitter,olteanu2014crisislex,alam2018crisismmd}, \datasetname{} covers a thousand different crisis events on a local scale. 
Unlike large-scale crisis events, most local events are not captured in knowledge sources such as Wikipedia. Accordingly, instead of being able to find relevant information from Twitter based on a set of event-dependent keywords, there is a need to design mechanisms for automatically detecting and tracking events directly from Twitter's stream. This is especially challenging due to the low number of available and related tweets for local events, which imposes a challenge for detecting those events as spikes or clusters~\cite{marcus2011twitinfo, hasan2018survey}.

% \iffalse
% \ke{not important, the data colletion part cover this with more details}
We create \datasetname{} in a two-step process applied to the public Twitter stream. First, we apply a knowledge-enhanced online clustering pipeline that generates noisy clusters of tweets related to each local event, and we manually select clusters as noisy timelines which contains interesting crisis event stories.   
Second, we recruit high-quality crowd-workers to refine selected clusters by extracting relevant, non-redundant, and informative tweets, to generate clean timelines. Annotators further write summaries to describe how the event progresses over time.  
% Finally, we propose 
% \fi

\datasetname{} supports two novel downstream tasks: timeline extraction and abstractive summarization. 
As shown in Figure \ref{fig:main-example}, the {\bf timeline extraction} task is formalized as, given a seed tweet as the initial mention of a crisis event, extracting relevant tweets with updates on the same event from the incoming noisy tweets stream. 
% The timeline correction task aims to facilitate research on creating concrete timelines of events by pruning out noisy and redundant information. Since the information on Twitter naturally contains lots of noise and redundancy~\cite{alam2021humaid}, 
This task is crucial for real-time event tracking. 
% This task differentiate from existing work on timeline generation ~\cite{yan2011evolutionary,tran2015timeline} 
% and preventing missing updates as relevant tweets are posted frequently.
% Here, we employ two post-processing steps to remove noise and redundancy as much as possible and later conduct an annotation task to clean the clusters even further.
The {\bf timeline summarization} task aims to
% facilitate research on 
generate abstractive summaries of evolving events by aggregating important details from temporal and incremental information. The summary tends to provide a quick and up-to-date overview to stakeholders (e.g., first responders) on what has been going on for the crisis event.
% from multiple sources~(i.e., tweets). 
Both tasks differentiate from existing work~\cite{mccreadie2018explicit,li2009enhancing,yan2011evolutionary,tran2015timeline}, where timeline extraction, generation, and summarization are often used interchangeably, where an extractive approach is used to identify a sequence of representative data points from a large corpus as the generated timeline or summary \ke{let me know whether this make sense to you all}. 
% Abstractive summarization necessitates the aggregation of incremental information, which is more challenging than the common extractive summarization~\cite{mccreadie2018explicit,li2009enhancing,yan2011evolutionary,tran2015timeline} task, where important data points are detected to be included in the summary. To the best of our knowledge, we are the first to deliver a relatively large dataset to benchmark abstractive summarization in the crisis domain. Additionally, compared to existing work on other domains~\cite{nallapati2016abstractive,narayan2018don,gusev2020dataset,gliwa2019samsum,kim2018abstractive}, summarizing timelines extracted from Twitter is more challenging due to the amount of noise~\cite{alam2021humaid}, the informal and noisy language, and the high overlap of information described in multiple tweets~\cite{rudra2018extracting}. Moreover, compared to centralized sources such as news~\cite{nallapati2016abstractive}, tweets can provide more frequent and real-time updates while covering various angles of an ongoing event.

% I think we can remove this paragraph
% The definition of a timeline \ke{we can move this part related work}\hossein{If we are going to keep this, let's keep it in intro because it highlights one important difference of our work with others and help clarify the contribution} in \datasetname{} is slightly different from the existing research on timeline generation~\cite{yan2011evolutionary,tran2015timeline}. Past research has mostly referred to the timeline as a retro-respective \ke{this is not correct, there are many online summarization work}\hossein{I am not talking about summarization, I am saying that timeline has been mostly reffered to as a retro-respective summarization to ..., so it is about what the timeline means in prior research.} summarization to provide an itemized report on an event. In \datasetname{}, a timeline is not a summary and includes every tweet containing updates on the event's progress. For instance, if we have the following two tweets in the chronological order of i) 2 people are injured and ii) 3 people are injured, both of these tweets are considered part of our timeline, while a summarization task would only take the second tweet.

\datasetname{} includes 1000 timelines with each one containing a unique crisis event. It mainly covers four domains including wildfire, local fire, traffic, and storm. To our best knowledge, this is the first timeline dataset focusing on ``local'' crisis events with the largest number of unique events \cite{10.1007/978-3-030-72113-8_33}. We collect \datasetname{} across seven states in the USA and two states of Australia, during 2020 and 2021. 
We further provide simple yet powerful baselines built on top of pretrained language models~(PLM) for each task. Our experiments show that there is still a considerable gap between the baseline models and the human performance, indicating the importance of this dataset for enabling future research on extracting clean and concrete crisis timelines and summarizing them. 

In summary, the contributions of this paper are as follows:
\begin{itemize}
    \item We propose \datasetname{}, which is the first dataset over clean and concrete local crisis event timelines
    \item We propose a novel cluster-then-refine approach to extract event timelines from public Twitter stream 
    \item We propose the first benchmark on abstractive timeline summarization in the crisis domain 
\end{itemize}

% In the remainder of this paper, we discuss the automated timeline generation in Section \ref{sec:generate}, the post-processing and annotation platform on generated timelines \ref{sec:correct}, and the baselines and experiments in Section \ref{sec:experiments}. 


==> sections/intro_second.tex <==
\section{Introduction}
We present \datasetname{}, the first dataset on extraction and summarization of local crisis event timelines from Twitter. An example of an annotated timeline in \datasetname{} is shown in Figure \ref{fig:main-example}. A timeline is a chronologically sorted set of posts, where each brings in new information or updates about an ongoing event. \datasetname{} supports two novel downstream tasks: \textbf{timeline extraction} and \textbf{timeline summarization}. 
As shown in Figure \ref{fig:main-example}, the {\bf timeline extraction} task is formalized as, given a seed tweet as the initial mention of a crisis event, extracting relevant tweets with updates on the same event from the incoming noisy tweets stream. This task is crucial for real-time event tracking. 
The {\bf timeline summarization} task aims to
generate abstractive summaries of evolving events by aggregating important details from temporal and incremental information. 
% The summary tends to provide a quick and up-to-date overview to stakeholders (e.g., first responders) on what has been happening during the crisis event.\hossein{The last sentence can be removed}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/intro_example.pdf}
\caption{This is a sample annotated timeline from \datasetname{}. The noisy timeline is the set of tweets sorted chronologically. The first tweet is the seed of the event. \cmark~means that the tweet is annotated to be part of the timeline and \xmark~indicates that the tweet is excluded from the timeline. The reason for exclusion is written under the mark.}
\label{fig:main-example}
\end{figure}

\datasetname{} can facilitate research in two directions 1) NLP for social good~(crisis domain) and 2) natural language generation~(summarization task). 
Here, we discuss the importance and the differences of \datasetname{} compared to previous work on each of these aspects.
% This is for the importance of humanitarian aid and our difference
Towards the first direction, the extraction of real-time crisis-relevant information from microblogs~\cite{zhang2019tracking,mamo2021fine} plays an important role in providing time-sensitive information to help first responders understand ongoing situations and plan relief efforts accordingly~\cite{sarter1991situation}. Existing research in this direction has mostly focused on extracting all crisis-relevant tweets about significant large-scale disaster events and mapping tweets to different categorizations such as humanitarian types~\cite{wiegmann2020disaster,imran2013practical,olteanu2014crisislex,imran2016twitter,alam2018crisismmd,alam2021crisisbench,alam2021humaid}.
% Recent research has heavily investigated this direction in both real-time~\cite{schulz2013see,rudra2018extracting,kumar2011tweettracker} and retrospective manner~\cite{repp2018extracting,alam2021crisisbench,alam2021humaid}. Existing datasets mainly focus on extracting all crisis-relevant tweets about significant large-scale disaster events and mapping them to humanitarian categories~\cite{wiegmann2020disaster,imran2013practical,olteanu2014crisislex,imran2016twitter,alam2018crisismmd,alam2021crisisbench,alam2021humaid}, actionable information~\cite{mccreadie2019trec}, or specific witness levels~\cite{zahra2020automatic}.
\datasetname{} goes beyond the simple task of categorizing each single post independently and enables a novel and more challenging task of extracting new updates of an ongoing crisis event from incoming posts. This can help provide time-sensitive updates while avoiding missing critical information in the bulk of the posts in microblogs due to the high volume of redundant and noisy information~\cite{alam2021humaid}. To the best of our knowledge, this is the first annotated dataset and evaluation benchmark for such extraction task while this problem has been tackled before in unsupervised settings~\cite{zhang2018geoburst}.

% is hard even for human due to the distributed nature of information in social media

% This is for local focus
Additionally, we focus on the extraction of \textbf{local} crisis events. The term ``local'' indicates that the event is bound to an exact location, such as a building, a street, or a county, and usually lasts for a short period. This is different from prior work that focused on large-scale and long-lasting crisis events affecting multiple and broader geographical areas. Consequently, although most existing datasets in crisis domain are limited to only tens of unique events \cite{imran2013practical,imran2016twitter,olteanu2014crisislex,alam2018crisismmd}, \datasetname{} covers a thousand different crisis events on a local scale. 
Unlike large-scale crisis events, most local events are not captured in knowledge sources such as Wikipedia. Therefore, instead of relying on finding relevant information from Twitter based on a set of event-dependent keywords, there is a need to design mechanisms for automatically detecting and tracking events directly from Twitter Stream. This is especially challenging due to the low number of available and related tweets for local events, which imposes a challenge for detecting such events as spikes or clusters~\cite{marcus2011twitinfo, hasan2018survey}, hence calling for clustering methods beyond mention-anomaly detection~\cite{asgari2021topic,guille2015event}. 

% challenges of making a concrete timeline and comparison with timeline generation
% The real-time extraction of concrete timelines for crisis events is closely related to the research on timeline generation~\cite{}, where an extractive approach is used to identify a sequence of representative data points from a large corpus to form an event timeline. Timeline generation has mostly been addressed as a retrospective and extractive summarization task~\cite{}, while \datasetname{} focuses on real-time extraction of any update in a time-sensitive setting. For instance, if we have the following two tweets in the chronological order of i) 2 people are injured and ii) 3 people are injured, both of these tweets are considered part of our timeline, while the extractive summarization approach would only take the second tweet.\hossein{May be we can just remove this section}

In the direction of natural language generation, \datasetname{} proposes a challenging task on abstractive timeline summarization. This task is challenging due to the need for aggregating information from multiple tweets~(compared to extractive summarization~\cite{yan2011evolutionary,tran2015timeline}) while considering temporal information. Compared to other sources of information~\cite{barros2019natsum,chen2019-ijcai}, summarizing Twitter timelines is more complicated due to the amount of noise~\cite{alam2021humaid}, the informal language~\cite{rudra2018extracting}, and the distributed nature of information compared to centralized sources such as news~\cite{nallapati2016abstractive}. \datasetname{} is the first dataset to provide human-written gold timeline summaries on the crisis domain or extracted information from Twitter in general.

% This task is essentially a more challenging multi-document summarization(MDS)~\cite{} as it requires further integration of temporal consideration in the summarization process. Lastly, \datasetname{} focuses on abstractive summarization. Except for a few~\cite{}, most of the prior research~\cite{} on timeline summarization has taken an extractive approach to form summaries by gathering representative sentences from important data points. The abstractive summarization task is more challenging due to the need for restructuring and generating new sentences to capture the important information. Compared to the existing abstractive summarization on other domains~\cite{}, summarizing Twitter timelines is more challenging due to the amount of noise~\cite{alam2021humaid}, the informal language~\cite{rudra2018extracting}, and the distributed nature of information compared to centralized sources such as news~\cite{nallapati2016abstractive}. \datasetname{} is the first dataset to provide human-written gold timeline summaries on the crisis domain or on top of Twitter in general.
We apply a two-step semi-automated process to the public Twitter stream to form 1000 local crisis timelines in \datasetname{}. This process is further described in Section \ref{sec:collection}. To our best knowledge, this is the first timeline dataset focusing on ``local'' crisis events with the largest number of unique events \cite{10.1007/978-3-030-72113-8_33}.

% We further evaluate simple yet powerful baselines from pretrained language models~(PLM) for each task. Our experiments show a considerable gap between the baseline models and human performance, indicating the importance of this dataset for enabling future research on extracting clean and concrete crisis timelines and summarizing them. 
% We create \datasetname{} in a two-step process applied to the public Twitter stream. First, we apply a noisy timeline collection pipeline that generates noisy clusters of tweets related to each local event. Second, we manually select clusters as noisy timelines which contain interesting crisis event stories.   
% Third, we recruit high-quality crowd-workers to refine selected clusters by extracting relevant, non-redundant, and informative tweets to generate clean timelines. Annotators further write summaries to describe how the event progresses over time.  
% Finally, we propose 
% \fi
% % from multiple sources~(i.e., tweets). 
% Both tasks differentiate from existing work~\cite{mccreadie2018explicit,li2009enhancing,yan2011evolutionary,tran2015timeline}, where timeline extraction, generation, and summarization are often used interchangeably, where an extractive approach is used to identify a sequence of representative data points from a large corpus as the generated timeline or summary \ke{let me know whether this make sense to you all}. 
% Abstractive summarization necessitates the aggregation of incremental information, which is more challenging than the common extractive summarization~\cite{mccreadie2018explicit,li2009enhancing,yan2011evolutionary,tran2015timeline} task, where important data points are detected to be included in the summary. To the best of our knowledge, we are the first to deliver a relatively large dataset to benchmark abstractive summarization in the crisis domain. Additionally, compared to existing work on other domains~\cite{nallapati2016abstractive,narayan2018don,gusev2020dataset,gliwa2019samsum,kim2018abstractive}, summarizing timelines extracted from Twitter is more challenging due to the amount of noise~\cite{alam2021humaid}, the informal and noisy language, and the high overlap of information described in multiple tweets~\cite{rudra2018extracting}. Moreover, compared to centralized sources such as news~\cite{nallapati2016abstractive}, tweets can provide more frequent and real-time updates while covering various angles of an ongoing event.
In summary, the contributions of this paper are as follows:
\begin{itemize}
    \item We propose \datasetname{}, which is the first dataset over clean and concrete local crisis event timelines
    \item We propose the first benchmark on abstractive timeline summarization in the crisis domain or on Twitter in general
    \item We provide the first dataset and evaluation benchmark, which goes beyond the tweet-level categorization of the crisis domain to facilitate research on real-time crisis even tracking.
    \item Our experiments show a considerable gap between the human performance and advance baseline models, indicating the importance of this dataset for enabling future research on extracting clean and concrete crisis timelines and summarizing them.
\end{itemize}

% In the remainder of this paper, we discuss the automated timeline generation in Section \ref{sec:generate}, the post-processing and annotation platform on generated timelines \ref{sec:correct}, and the baselines and experiments in Section \ref{sec:experiments}. 

